ATHENA Detector Proposal -- A Totally Hermetic Electron Nucleus Apparatus proposed for IP6 at the Electron-Ion Collider

ATHENA has been designed as a general purpose detector capable of delivering the full scientific scope of the Electron-Ion Collider. Careful technology choices provide fine tracking and momentum resolution, high performance electromagnetic and hadronic calorimetry, hadron identification over a wide kinematic range, and near-complete hermeticity. This article describes the detector design and its expected performance in the most relevant physics channels. It includes an evaluation of detector technology choices, the technical challenges to realizing the detector and the R&D required to meet those challenges.

==> Detector/challenges_pid.tex <==
%\begin{table}[p]
\centering
%\footnotesize
\scriptsize
%\tiny
\renewcommand{\arraystretch}{1.4}
%\begin{tabular}{|p{1.75cm}|p{4cm}|p{4cm}|p{4cm}|}
\caption{Challenges and mitigation policies for particle identification technologies.}
\label{tab:pid}
\begin{tabular}{|p{1.5cm}|p{4cm}|p{8cm}|p{7cm}|}
%
%   Header
%
\hline
\multicolumn{4}{|c|}{\textbf{Particle Identification}} \\ \hline
\rowcolor[gray]{.9}
\multicolumn{1}{|c}{Component} &
\multicolumn{1}{|c}{Technology} &
\multicolumn{1}{|c}{Maturity} &
\multicolumn{1}{|c|}{Alternatives \& Mitigation} \\
\hline \hline
%
%   Data
%
dRICH (forward), global design &
Combination of gas and aerogel in large acceptance focusing  RICH in magnetic field. &
Two-radiator RICHs already operated in experiments (HERMES, LHCb). The specific radiator combination in relation with the expected environment at EIC to be validated. \textbf{Maturity Level of the Technology: 9}  &
Completion of the ongoing studies by prototyping and test beam runs.  \\
\hline
%
hpDIRC (barrel), global design &
DIRC concept empowered by focusing element and fine-pixel readout. &
Focusing DIRC extensively developed and confirmed by test beam for PANDA at GSI. Principle of hpDIRC (more refined focusing by lenses) demonstrated with optical studies. Confirmation of the performance of the hpDIRC needed. \textbf{Maturity Level of the Technology: 9}  &
Completion of the ongoing studies by prototyping and test beam runs.  \\
\hline
%
pfRICH (backward), global design &
Proximity focusing RICH with aerogel radiator and large proximity gap for fine resolution. &
Proximity focusing demonstrated in various experiments (ALICE, BELL II); aerogel as RICH radiator demonstrated (HERMES, LHCb, BELLE II, CLAS12). Confirmation of the performance of the pfRICH needed. \textbf{Maturity Level of the Technology: 9} &
Completion of the simulation studies specific to EIC. \\
\hline
%
Photosensors by SiPMs (for dRICH and pfRICH) &
SiPMs at low temperature ($\sim -40^\circ$~C). &
The validation of the approach is via a dedicated  R\&D program including the study of the dark current versus irradiation dose and versus repeated thermal annealing cycles; SiPM selection by characterizing devices by different providers; highly innovative approach. \textbf{Maturity Level of the Technology: 6}  &
Continue pursuing the development of an alternative approach by large-size MCP devices: LAPPDs; as both the baseline choice (SiPM)  and the alternative option (LAPPD) are not established, both items require management attention, adequate support, and investment.  \\
\hline
%
Photosensors by MCP-PMTs (for hpDIRC) &
Commercial 1-inch MPC-PMTs (most likely by \it{Photonis}). & Challenges arise from the
production rate and cost. The use of the technology in high magnetic field that can reduce the gain and, therefore, the time resolution needs to be confirmed. \textbf{Maturity Level of the Technology: 9} &
Early purchasing procedure. Further studies of performance in realistic magnetic field.
Fallback option:
continue pursuing the development of an alternative approach by large-size MCP devices (LAPPD).   \\
\hline
%
%
Radiator gas (for dRICH) &
C$_2$F$_6$. &
Procurement difficulties and increasing cost because of increasing usage restrictions (worldwide) related to the extremely high \gls{gwp}).  Recirculation plant required. \textbf{Maturity Level of the Technology: 7} &
Fallback option: Develop the approach by pressurized Argon to replace the use of fluorocarbon gas.   \\
\hline
%
Aerogel (for dRICH and pfRICH) &
Low refractive index (1.02) aerogel &
The homogeneity and yield in the production of hydrophobic or hydriphilic low refractive index aerogel has to be demonstrated as well as the production rate.  \textbf{Maturity Level of the Technology: 7} &
Develop the low refractive index aerogel together with more than a single producer
(University of Chiba, Japan, Budker Institute, Russia, and  \it{ASPEN AEROGELS, INC.}, USA where aerogel development is supported by a SBIR grant); early purchasing.    \\
\hline
%
Synthetic fused silica bars (for hpDIRC) &
Synthetic fused silica bars with high precision mechanical parameters and very fine surface polishing; re-use of BaBar material expected. &
A detailed protocol for BaBar silica bar disassembly to be established; a protocol for barrel assembly in ATHENA needs to be put in place. \textbf{Maturity Level of the Technology: 9} &
Guidance from BaBar and PANDA experience.  \\
\hline
%
Barrel TOF  &
Sensors: \gls{aclgad}. &
Dedicated development, already advanced at the present time; synergies with other proposed applications: ATLAS roman pots for HL-LHC, LHCb upgrade, ALICE3, NA62 (CERN), PIENUX  (TRIUMF), and PAN space missions. \textbf{Maturity Level of the Technology: 8}  &
Continue pursuing the development of an alternative approach for PID at low momenta to complement PID by DIRC in the barrel: R\&D dedicated to a miniTPC with sensors by GridPix technology.  \\
\hline
%
\end{tabular}
%\end{table}
